Learn from Balance: Rectifying Knowledge Transfer for Long-Tailed Scenarios

Knowledge Distillation (KD) transfers knowledge from a large pre-trained teacher network to a compact and efficient student network, making it suitable for deployment on resource-limited media terminals. However, traditional KD methods require balanced data to ensure robust training, which is often unavailable in practical applications. In such scenarios, a few head categories occupy a substantial proportion of examples. This imbalance biases the trained teacher network towards the head categories, resulting in severe performance degradation on the less represented tail categories for both the teacher and student networks. In this paper, we propose a novel framework called Knowledge Rectification Distillation (KRDistill) to address the imbalanced knowledge inherited in the teacher network through the incorporation of the balanced category priors. Furthermore, we rectify the biased predictions produced by the teacher network, particularly focusing on the tail categories. Consequently, the teacher network can provide balanced and accurate knowledge to train a reliable student network. Intensive experiments conducted on various long-tailed datasets demonstrate that our KRDistill can effectively train reliable student networks in realistic scenarios of data imbalance.

==> _Related_works.tex <==
\subsection{Knowledge Distillation}
Knowledge distillation aims to train a lightweight and accurate student network by mimicking the informative knowledge of a powerful yet cumbersome teacher network.
Existing knowledge distillation methods can be categorized into three groups based on the type of knowledge transferred by the teacher network, including logit-based, feature-based, and relation-based.
Among them, the logit-based methods~\cite{Hinton2015,zhao2022decoupled} propose to soft or decouple the predictions of the teacher network to provide expressive supervision signals to the student network. 
On the other hand, feature-based methods~\cite{romero2014fitnets,zagoruyko2016paying,chen2021distilling} find that high-dimensional features of the teacher network contain more information than low-dimensional logits. 
Therefore, they transfer the meaningful middle-layer attention features or representations from the teacher network to improve the performance of the student network. 
Instead of directly transmitting the logits or features output by the teacher network, relation-based distillation methods~\cite{tung2019similarity,park2019relational} explore instance-level or category-level relations as a form of knowledge. 
As a result, the student network that effectively mimics these relations of the teacher network can produce representations similar to those of the teacher network.

While the aforementioned methods excel in training reliable student networks on balanced standard datasets, they face challenges when applied to real-world imbalanced data. 
Figure~\ref{fig1} (a) illustrates the class imbalance issue, where the majority of examples belong to head categories, leaving few examples for other categories. 
This imbalance biases the teacher network towards head categories, leading to suboptimal student network performance.
To mitigate the impact of imbalanced data on the distillation effect, we modify the imbalanced feature representations and logits of the teacher network to enhance the performance of the student network. 

\subsection{Long-Tailed Learning}

Long-tailed learning methods aim to alleviate the issue encountered in data imbalance scenarios, where the model tends to overly focus on the head classes, resulting in poor performance on the tail classes. 
Existing long-tailed learning methods mainly leverage re-sampling, re-weighting, and multi-expert methods to mitigate data imbalances and ensure reliable model performance.
Re-sampling methods provide relatively balanced data to the model by oversampling the tail classes~\cite{pouyanfar2018dynamic} or undersampling the head classes~\cite{buda2018systematic}.
The re-weighting~\cite{cui2019class,cao2019learning} methods enhance the influence of tail class examples on model gradient updates by increasing the weight of tail class examples.
% The multi-expert methods~\cite{xiang2020learning,wang2020long} employ model learning from multiple expert models, which extract knowledge from imbalanced data by considering various perspectives.  
These methods effectively solve the interference of imbalanced data in the model optimization process.

In this paper, we consider the imbalanced knowledge from the teacher network as a crucial supervisory signal for optimizing the student network in knowledge distillation.
Recent works reduce bias in the knowledge provided by the teacher network by weighting~\cite{he2023joint,zhang2023balanced} and softening~\cite{he2021distilling} teacher predictions.
However, unbalanced representations and misclassified predictions of the teacher network are still ignored despite their potential to mislead student networks.
Therefore, we propose the KRDistill to rectify the imbalanced feature representations and misclassified predictions from the teacher network, and transfer clear and balanced knowledge to learn a reliable student network.

